Understanding and Mitigating Multi-Sided Exposure Bias in Recommender Systems

Fairness is a critical system-level objective in recommender systems that has been the subject of extensive recent research. It is especially important in multi-sided recommendation platforms where it may be crucial to optimize utilities not just for the end user, but also for other actors such as item sellers or producers who desire a fair representation of their items. Existing solutions do not properly address various aspects of multi-sided fairness in recommendations as they may either solely have one-sided view (i.e. improving the fairness only for one side), or do not appropriately measure the fairness for each actor involved in the system. In this thesis, I aim at first investigating the impact of unfair recommendations on the system and how these unfair recommendations can negatively affect major actors in the system. Then, I seek to propose solutions to tackle the unfairness of recommendations. I propose a rating transformation technique that works as a pre-processing step before building the recommendation model to alleviate the inherent popularity bias in the input data and consequently to mitigate the exposure unfairness for items and suppliers in the recommendation lists. Also, as another solution, I propose a general graph-based solution that works as a post-processing approach after recommendation generation for mitigating the multi-sided exposure bias in the recommendation results. For evaluation, I introduce several metrics for measuring the exposure fairness for items and suppliers, and show that these metrics better capture the fairness properties in the recommendation results. I perform extensive experiments to evaluate the effectiveness of the proposed solutions. The experiments on different publicly-available datasets and comparison with various baselines confirm the superiority of the proposed solutions in improving the exposure fairness for items and suppliers.

==> Chapters/BiasInRS_02.tex <==
\chapter{Fairness in Recommender Systems}
\label{chap:biasinrs}
\tikzsetfigurename{biasinrs_}

\section{Introduction}

\subsection{Fairness definitions}
\subsection{Metrics for evaluation fairness in recommendations}

\section{Factors leading to unfair recommendations}

\section{Impacts of unfair recommendations}

% As I mentioned earlier, recommender systems often operates in a multi-sided environment where different stakeholders or entities are involved in the system: user, item, and suppliers \cite{burke2016,abdollahpouri2019beyond,burke2017b}. Satisfying the needs and utilities of each entity is key for achieving fairness in recommender systems. Unfair recommendation can adversely impact the satisfaction and utility of each entity. 

% In item-side, unfair distribution of recommended items can amplify the \textit{popularity bias}: a few popular items are frequently recommended, while majority of unpopular items are rarely recommended \cite{steck2011item,ciampaglia2018algorithmic,abdollahpouri2020multi,park2008long,Jannach2015,longtailnichesriche}. In this situation, popular items would be over-recommended even more that their merit in the rating data and unpopular items would be less recommended. This skew in the frequency of recommended items in recommendation lists not only  adversely impact the whole ecosystem, but also negatively affects the experience of both suppliers (some suppliers may not receive enough attention) \cite{abdollahpouri2020unfair} and users (those who are not interested in popular items still receive popular items in their recommendations) \cite{himan2019b}.  

% Tendency of recommendation systems on more recommending popular items will cause the recommendation lists mainly consist of items that belong to few suppliers which would be unfair towards other suppliers, evidencing supplier-side unfairness. Unfair treatment of suppliers may cause the items belong to some suppliers frequently appear in the recommendation lists, while the items belong to the other suppliers do not receive the proportionate attentions. This skewness in the appearance of suppliers in recommendation lists may stimulate those suppliers to leave the system which will have negative impact on the whole system in long run \cite{abdollahpouri2020unfair,abdollahpouri2020multi,surer2018,mehrotra2018towards}.

% Finally, user-side unfairness not only perpetuates undesirable social dynamics, it can also degrade the satisfaction of certain groups of users. Measuring user-side fairness is a challenging task and requires online evaluation of recommendation lists on a real-world platform with steady stream of data which is not always available. But, in an offline setting, it can be simply defined as any disparity in the quality of recommendation generated for the users. For instance, if group $A$ receives recommendations which are consistently better matched with their preferences than those of group $B$, it shows that the recommendation algorithm mainly learned the preferences of group $A$, showing algorithmic bias against group $B$ \cite{ekstrand2018}. 

% In this thesis, we seek to mitigate exposure bias of items and suppliers while recommending relevant and accurate items to the users.

\section{Techniques for addressing unfair recommendations}

==> Chapters/BiasMitTechs.tex <==
\chapter{Bias mitigation techniques and their limitations}
\label{chap:BiasMitTechs}
\tikzsetfigurename{biasmittechs_}

\section{Bias mitigation techniques}

The concept of popularity bias has been studied by many researchers often under different names such as long-tail recommendation \cite{abdollahpouri2017controlling,yin2012challenging}, Matthew effect \cite{moller2018not}, and aggregate diversity \cite{liu2015trust,adomavicius2011improving} all of which refer to the fact that the recommender system should recommend a wider variety of items across all users. 


The solutions for tackling popularity bias in the literature can be categorized into two groups:\footnote{A third option, preprocessing, is generally not useful for popularity bias mitigation because undersampling the popular items greatly increases the sparsity of the data.} \textit{Model-based} \cite{vargas2014improving,sun2019debiasing,abdollahpouri2017controlling,adamopoulos2014over} and \textit{re-ranking} \cite{adomavicius2011maximizing,adomavicius2011improving,antikacioglu2017,abdollahpouri2019managing}. In model-based solutions the recommendation generation step is modified, so that the popularity of the items is taken into account in the rating prediction. For example authors in \cite{abdollahpouri2017controlling} proposed a regularization term to control the popularity of recommended items that could be added to an existing objective function of a learning-to-rank algorithm \cite{karatzoglou2013learning} to improve the aggregate diversity of the recommendations. In another work, Vargas and Castells in \cite{vargas2011rank} proposed probabilistic models for improving novelty and diversity of recommendations by taking into account both relevance and novelty of target items when generating recommendation lists. Moreover, authors in  \cite{vargas2014improving}, proposed the idea of recommending users to items for improving novelty and aggregate diversity. They applied this idea to nearest neighbor models as an inverted neighbor and a factorization model as a probabilistic reformulation that isolates the popularity components. 

In the second approach for improving aggregate diversity, the algorithm takes a larger output recommendation list and re-orders the items in the list to extract a shorter final list with improved long-tail properties. Most of the solutions for tackling popularity bias fall into this category. For example, Adomavicius and Kwon \cite{adomavicius2011maximizing} proposed the idea of diversity maximization using a maximum flow approach. They used a specific setting for the bipartite recommendation graph in a way that the maximum amount of flow that can be sent from a source node to a sink node would be equal to the maximum aggregate diversity for those recommendation lists. In their setting, given the number of users is $m$, the source node can send a flow of up to $m$ to the left nodes, left nodes can send a flow of up to 1 to the right nodes, and right nodes can send a flow of up to 1 to the sink node. Since the capacity of left nodes to right nodes is set to 1, thus the maximum possible amount of flow through that recommendation bipartite graph would be equivalent to the maximum aggregate diversity. 

A more recent graph-based approach for improving aggregate diversity which also falls into the reranking category was proposed by Antikacioglu and Ravi in \cite{antikacioglu2017}. They generalized the idea proposed in \cite{adomavicius2011maximizing} and showed that the minimum-cost network flow method can be efficiently used for finding recommendation subgraphs that optimizes the diversity. In this work, an integer-valued constraint and an objective function are introduced for discrepancy minimization. The constraint defines the maximum number of times that each item should appear in the recommendation lists and the objective function aims to find an optimal subgraph that gives the minimum discrepancy from the constraint. This work shows improvement in aggregate diversity of the items with a smaller accuracy loss compared to the work in \cite{vargas2011rank} and \cite{vargas2014improving}. Our algorithm is also a graph-based approach that not only is it able to improve aggregate diversity and the exposure fairness of items, it also gives the suppliers of the recommended items a fairer chance to be seen by different users. Moreover, unlike the work in \cite{antikacioglu2017} which tries to minimize the discrepancy between the distribution of the recommended items and a target distribution, our FairMatch algorithm has more freedom in promoting high-quality items or suppliers with low visibility since it does not assume any target distribution of the recommendation frequency.

Another work that also uses a re-ranking approach is by Abdollahpouri et al. \cite{abdollahpouri2019managing} where authors proposed a diversification method for improving aggregate diversity and long-tail coverage in recommender systems. Their method was based on \textit{eXplicit Query Aspect Diversification} (xQuAD) algorithm \cite{santos2010exploiting} that was designed for diversifying the query result such that it covers different aspects related to a given query. In \cite{abdollahpouri2019managing}, the authors used xQuAD algorithm for balancing the ratio of popular and less popular (long-tail) items in final recommendation lists. 

In addition, in \cite{fairmatch2020umap}, we proposed a graph-based algorithm that finds high quality items that have low visibility in the recommendation lists by iteratively solving the maximum flow problem on recommendation bipartite graph. The present work extends the idea in \cite{fairmatch2020umap} for improving the exposure fairness of items and suppliers. We also discuss the limitations of existing metrics for measuring the exposure bias in recommendation results and propose several metrics to overcome those limitations. 

In addressing exposure bias in domains like job recommendations where job seekers or qualified candidates are recommended, Zehlike et. al. \cite{zehlike2017fa} proposed a re-ranking algorithm to improve the ranked group fairness in recommendations. 
%This method was originally used for improving group fairness in job recommendation. 
The algorithm creates queues of protected and unprotected items and merges them using normalized scoring such that protected items get more exposure. 

%In their setting, a recommendation set of candidates satisfies the ranked group fairness criterion if it fairly represents candidates belong to the protected group, contains the most qualified candidates, and orders the candidates based on their qualification (more qualified candidates should appear on top of the recommendation set). The fair representation of protected candidates in a recommendation list is determined by comparing the number of protected candidates in the ranked list and the expected number of candidates if they were selected at random. The algorithm optimizes to re-rank the candidates to achieve the fair representation of protected candidates in recommendation lists while considering the qualification of the candidates.



% This method was originally used for improving group fairness in job recommendation and was adapted here to improve the fairness of recommendations in terms of head versus long-tail items in recommendations. The algorithm creates queues of protected and unprotected items and merges them using normalized scoring such that protected items get more exposure.


Most of the existing works in the literature for improving aggregate diversity and exposure fairness have only concentrated on the items and ignored the fact that in many recommendation domains the recommended items are often provided by different suppliers and hence their utility should also be investigated. To the best of our knowledge, there are only few prior works that have addressed this issue such as \cite{abdollahpouri2020addressing} and \cite{mehrotra2018towards}. In \cite{abdollahpouri2020addressing}, authors illustrated how popularity bias is a multistakeholder problem and hence they evaluated their solution for mitigating this bias from the perspective of different stakeholders. Mehrotra et al. \cite{mehrotra2018towards} investigated the trade-off between the relevance of recommendations for users and supplier fairness, and their impacts on users' satisfaction. Relevance of the recommended items to a user is determined by the score predicted by a recommendation algorithm. To determine the supplier fairness in recommendation list, first, suppliers are grouped into several bins based on their popularity in rating data and then the supplier fairness of a recommendation list is measured as how diverse the list is in terms of covering different supplier popularity bins. 

Our work in this paper also observes the importance of evaluating algorithms from the perspective of multiple stakeholders and we propose an algorithm that can directly improve the visibility of the suppliers without losing much accuracy from the users' perspective.

\section{Limitations of existing bias mitigation techniques}

Various algorithmic solutions have been proposed to tackle the unfairness in recommender systems. However, there are several limitations in those solutions. In this section, we discuss the limitations of existing solutions for addressing unfairness in recommender systems.

First, a large body of existing solutions has one-sided view on addressing the unfairness of recommendation systems, meaning that they optimize to improve the fairness of one entity, overlooking the fairness of other entities in the system. For example, research works in \cite{burke2017,edizel2020,zehlike2017fa,ekstrand2012,yao2017,ekstrand2018} optimize for user-side fairness or research works in \cite{abdollahpouri2019managing,wang2016multi,recsys2017,antikacioglu2017,vargas2014improving,adomavicius2011maximizing,vargas2011} only optimize for item-side fairness. Although these works showed improvement on one side, it is not clear how they are affecting other sides, most likely those approaches adversely affected the other sides of the system . It has been shown that only improving the fairness of one side will hurt the fairness of the other sides \cite{mehrotra2018towards}.   

Second, existing solutions with multi-sided view usually optimize to generate a list of recommendations for each user to contain items from different suppliers while maintaining the relevance of items for each user \cite{mehrotra2018towards,suhr2019two}. In these approaches, the proposed models optimize to locally improve the supplier fairness for the list generated for one user in the hope that improving supplier fairness separately for a user's list results in global optimum for the whole recommendation lists. However, we argue that optimizing for supplier fairness requires a holistic view over the whole recommendation lists, not the recommendation list for a user. For instance, consider a recommendation algorithm that recommended 10 items from 10 different suppliers to each user. In this situation, the recommendation list for each user will have items from different suppliers, while the overall recommendation lists only have items from 10 suppliers which is unfair against other suppliers. Thus, it is important to keep track of supplier fairness over the whole recommendation lists. 
\todo[inline]{A figure should be added.}

Third, some of the existing solutions are designed to specifically address the fairness in a domain and cannot be generalized to fairness definitions of other domains \cite{mehrotra2018towards,yao2017,steck2018calibrated}. 

For example, Mehrota et al., in \cite{mehrotra2018towards} used equality of attention as the utility of supplier and the relevance score of target item predicted by the base recommender for target user as the utility of users. However, fairness is a general concept and may have different definitions depending on the application and the domain under study. Therefore, a flexible algorithmic solution with capability of being generalized for different notion of fairness is needed.

==> FrontBackMatter/Dedication.tex <==
% Version 1.0 by Joos Buijs, Eindhoven, August 2014
% Use at your own risk.
% Attribution is appreciated 

%*******************************************************
% Dedication
%*******************************************************
\thispagestyle{empty}
\clearpage

\par\vspace*{.35\textheight}{\centering Dedication\ldots\par}


==> Tables/6.3.1.flatness.tex <==
\captionsetup[table]{skip=4pt}
\begin{table}[t!]
\small
\centering
\captionof{table}{Flatness ($\mathcal{F}$) and kurtosis ($\mathcal{K}$) of rating distribution} \label{tab:flatness}
\begin{tabular}{llrrrr}
\toprule
 Dataset & method & rating & z-score & $\mbox{Per}^f_u$ & $\mbox{Per}^l_u$ \\ 
 \midrule
 \multirow{2}{*}{MovieLens} & $\mathcal{F}$ & 0.154 & 0.450 & 0.100 & 0.101 \\
                       & $\mathcal{K}$ & 2.644 & 3.132 & 2.151 & 1.988 \\
\cline{1-6}
 \multirow{2}{*}{Goodreads} & $\mathcal{F}$ & 0.269 & 0.425 & 0.070 & 0.140 \\
                       & $\mathcal{K}$ & 2.906 & 2.893 & 2.004 & 2.019 \\
\bottomrule
\multicolumn{6}{l}{\textit{Flatness of a uniform distribution is $\mathcal{F}=0$.}} \\
\multicolumn{6}{l}{\textit{Kurtosis of a uniform distribution is $\mathcal{K}<3$.}} \\
\end{tabular}
\end{table}

